Agentic DAG-Orchestrated Planner Framework for Multi-Modal, Multi-Hop Question Answering in Hybrid Data Lakes

Enterprises increasingly need natural language (NL) question answering over hybrid data lakes that combine structured tables and unstructured documents. Current deployed solutions, including RAG-based systems, typically rely on brute-force retrieval from each store and post-hoc merging. Such approaches are inefficient and leaky, and more critically, they lack explicit support for multi-hop reasoning, where a query is decomposed into successive steps (hops) that may traverse back and forth between structured and unstructured sources. We present Agentic DAG-Orchestrated Transformer (A.DOT) Planner, a framework for multi-modal, multi-hop question answering, that compiles user NL queries into directed acyclic graph (DAG) execution plans spanning both structured and unstructured stores. The system decomposes queries into parallelizable sub-queries, incorporates schema-aware reasoning, and applies both structural and semantic validation before execution. The execution engine adheres to the generated DAG plan to coordinate concurrent retrieval across heterogeneous sources, route intermediate outputs to dependent sub-queries, and merge final results in strict accordance with the plan's logical dependencies. Advanced caching mechanisms, incorporating paraphrase-aware template matching, enable the system to detect equivalent queries and reuse prior DAG execution plans for rapid re-execution, while the DataOps System addresses validation feedback or execution errors. The proposed framework not only improves accuracy and latency, but also produces explicit evidence trails, enabling verification of retrieved content, tracing of data lineage, and fostering user trust in the system's outputs. On benchmark dataset, A.DOT achieves 14.8% absolute gain in correctness and 10.7% in completeness over baselines.

==> framework.tex <==
\section{Framework}
\label{sec:ps}


% \subsection{Problem Formulation}
% \label{sec:tf}

% Consider a hybrid data lake consisting of a structured relational database $\mathbf{D_S}$ and an unstructured document collection $\mathbf{D_U}$. 
% The hybrid data lake $\mathbf{D} = \{D_S, D_U\}$.
% The database $\mathbf{D_S}$ is represented as a set of tables:
% \[
% \mathbf{D_S} = \{ T_1, T_2, \dots, T_m \},
% \]
% where each table $T_i$ has a schema with columns 
% \[
% C_{i,1}, C_{i,2}, \dots, C_{i,k}
% \]
% and rows 
% \[
% R_{i,1}, R_{i,2}, \dots, R_{i,n}.
% \]

% The document collection $\mathbf{D_U}$ consists of unstructured text documents:
% \[
% \mathbf{D_U} = \{ d_1, d_2, \dots, d_p \}.
% \]

% Each document ${d_i}$ from $D_U$, is linked to one or more rows with a table $T_j$ in $\mathbf{D_S}$ via foreign keys or metadata tags. This enables seamless traversal between structured and unstructured data.

% Given a natural language question Q, the system must retrieve evidence from both $D_S$ and $D_U$  and generate an answer $Ans$ that synthesizes information across modalities, using both tables and texts for coherent final response.


% \subsection{Solution Overview}
% \label{subsec:overview}

% We propose A.DOT, an end-to-end agentic architecture with modular components to answer a natural langugae query over a hybrid data lake. The system comprises four core components Figure \ref{fig:main_framework}: First, a Plan Generator breaks down the complex question into a Directed Acyclic Graph (DAG) styled subquestions. Next, a dual-validation system (Syntactic Validator and Semantic Validator) checks whether the nodes in the DAG comply with the schema, returning a well-defined plan to the execution engine which attempts to execute the tasks using downstream datasources. There could be a chance where the DAG plan produced by the Plan generator mismatches with the structure or the database schema and to solve this issue we introduce the Re-Planner, which refine and repair the plan based on the specific parameters provided through a limited time iteration. For the given DAG, the Executor triggers parallel independent queries following the DAG structure while preserving variable dependencies across nodes and produces the correct aggregation of results to produce the final answer. Using the previously successful computational plans, we cache them using Plan Caching to save time and computational cost, by applying advanced intelligent caching strategies.
% \begin{figure*}[ht!]
%     \centering
%     \includegraphics[width=\textwidth]{figures/iaai-Middle Level Diagram.png}
%     \caption{The Overall Framework}
%     \label{fig:main_framework}
% \end{figure*}



% \subsection{Database Construction}
% \label{subsec:db_construction}

% To operationalize the hybrid data lake $D$ = $\{D_S, D_U\}$, we store the structured component $D_S$ = ${T_1, T_2, . . . , T_m}$ in a relational SQL database, where each table $T_j$ retains its schema with columns $C_{i1},... , C_{ik}$ and rows $R_{i1},... , R_{in}$. For unstructured documents $D_U$ = $\{d_1,d_2,... , d_p\}$, we employ a chunking pipeline to segment each document into smaller, semantically coherent units, which are then embedded using a pre-trained sparse and dense embedding model. The resulting chunk embeddings are stored in Milvus, a scalable vector database that enables fast similarity search. The embedded chunks are represented as $VU$ =$\{v_1,v_2,.. ,v_q\}$, where each $v_i$ is an attribute-rich vector comprising: (i) the chunk text, (ii) metadata (e.g., source document ID, timestamp), and (iii) a dense vector embedding for semantic comparison. and (iv) a sparse vector embedding for sparse retriever.

% We define, a \textbf{database schema} $\mathbf{S}$ defines the high-level structure of both $\mathbf{D_S}$ and $\mathbf{D_u}$, including:
% \begin{itemize}
%     \item \textbf{Table schemas}: Column names, data types, primary/foreign keys, and constraints (e.g., NOT NULL).
%     \item \textbf{Vector store specifications}: The Milvus collection structure, with metadata and linkage fields (e.g., document\_id, table\_name, row\_id).
%     \item \textbf{Connection Details}: how chunks from the vector store connect to a column of a table in the structured database.
% \end{itemize}

% \subsection{Plan Caching}
% \label{subsec:plan_caching}

% To accelerate query processing and reduce the latency of repeated or semantically similar questions, we introduce the Plan Caching Module, a retrieval-augmented component that stores validated plans and enables fast reuse during inference. This module is motivated by the observation that, in enterprise environments, users often issue repetitive queries with minor variations to extract similar information from the hybrid data lake. Generating a fresh plan for each query—via the plan generator module—incurs unnecessary LLM invocations and computational overhead. The Plan Caching Module mitigates this by maintaining a strategic plan repository indexed by the database schema and query, thereby reusing validated plans that align with a user’s current request.

% The repository is structured to user questions $Q$ = $\{q_1,q_2,... ,q_k\}$ along with the corresponding database schema $S$ = $\{S_1, S_2, ...S_k \}$ to previously validated plans $P$ = $\{p_1,p_2,... ,p_k\}$. We also use the database schema along with each query for caching, because the plan can differ for the same query based on the database schema $S$ ,  To accommodate various query matching criteria, we implement three caching strategies:

% 1. Exact Caching – The user question q is checked for a verbatim match against the set of cached queries Q. If found, the corresponding plan pi is retrieved and executed directly. This is deterministic and lightweight but limited to identical queries.

% 2. Semantic Caching – Leverage Natural Language Inference (NLI) models to assess whether the user’s question entails or matches any stored question $q_i \in Q$ in semantic meaning. This enables the retrieval of a semantically equivalent plan even when the phrasing or syntax differ.

% 3. Template-Based Caching – Predefined templates are stored in parameterized form, with variable placeholders representing entity slots (e.g., “Find the {placeholder} for customers in Texas”). Incoming questions are matched against templates; if a match is detected, the cached plan is instantiated with the current placeholder values. This approach handles parametric queries efficiently.

% To manage memory and retrieval speed, we adopt an LRU (least-recently-used) caching policy with a configurable capacity (e.g., up to 1,000 query-schema pairs). When a cache hit occurs, the retrieved plan bypasses the plan generator and propagates directly to the Plan Executor Module. If no plan is found, the plan generator receives the query and schema, and the resulting plan is stored in the cache upon validation.

% Further, at the moment the cache is considering at query level, but considering at “subquery-level” could lead to identifying the query that partially resembles the stored query and extract the corresponding subplan, but we left it as a future research direction.

% By implementing the Plan Caching Module, we improve system responsiveness and reduce redundant computation, making A.DOT suitable for real‑time enterprise deployments.

% \subsection{Plan Generator}
% \label{subsec:plan_generator}

% % This is the core section where i will be explaining the plan structure its inputs and outputs, what is the hard problems in this, why DAG is needed compared to the direct iterative decomposition and how the variable dependencies are being used to maintain the dependencies between the subqueries, and what are the other attributes in a node like should\_expose\_answer that helps to reduce the amount of time the waiting for the answer, by showing the intermediate answer like streaming and finally compiling all the necessary subqueries answer to get the final answer.

% The Plan Generator Module serves as the core orchestration engine of A.DOT, responsible for decomposing a user’s natural-language query Q into an executable directed acyclic graph (DAG) in a single shot. Unlike prior agentic frameworks such as ReAct or Plan-and-Solve, which iteratively invoke an LLM to process intermediate sub-query outputs, our module produces a static, self-contained plan that encodes all the sub-tasks and their dependencies up front. This DAG-first approach incurs lower latency, avoids the overhead of repeated LLM calls per sub-query, and prevents cascading errors that can arise from localized reasoning steps.

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.4\textwidth]{figures/iaai-Plan_Generator.png}
%   \caption{An DAG Plan Demonstration}
%   \label{fig:dag_plan}
% \end{figure}

% Each user query $Q$ is decomposed into atomic sub-queries that map to operations over $D_S$ (structured database) or $D_U$ (document collection). The generated plan is represented as a DAG of the form $G = (V, E)$, where:

% $V = {n_1, n_2, ..., n_k}$: nodes corresponding to sub-queries (operational units)
% $E = {e_1, e_2, ..., e_i}$: edges representing dependency relationships
% Each node $n_i \in V$ is a sub-query with the following attributes:

% 1. Subquery (question) – A specific operation (e.g., retrieval, aggregation)
% Tool – the target data source (iceberg for SQL, Milvus for document collection vectors). It also includes the dependency variable information that needs to be handled during the execution.

% 2. Label – a variable that stores the result of $n_i$

% 3. Should\_expose\_answer – A Boolean flag: If true, the result of the sub-query execution is immediately returned to the user as a partial answer, without waiting for the full execution across the DAG.

% The edges $e_i \rightarrow e_j \in E$ capture dependency relationships, where the output of $n_i$ is required as an input to $n_j$.

% An example of this is shown in the figure \ref{fig:dag_plan}. Furthermore, the should\_expose\_answer flag is designed to minimize perceived latency and maximize intermediate visibility into the end user. Since in some cases the intermediate sub-queries can partially answer the user query, which is shown to the user, this ensures that the partial result is relayed back to the user without forcing them to wait on the entire DAG scope.

% \subsection{Plan Validator}
% \label{subsec:plan_validator}

% The Plan Validator Module ensures that the generated DAG plan is structurally and semantically coherent before execution, providing a correctness guarantee that minimizes downstream errors. The goal of plan validation is to verify that the plan respects the schema, dependencies, and query constraints. We define the validation procedure as:

% $V: (P,S) \rightarrow (correct, feedback)$

% where: $P$ is the DAG plan, $S$ is the database schema, $correct$ is a Boolean flag indicating plan correctness and $feedback$ is the actionable feedback for the violations of rules for invalid plans.

% The Plan Validator intervenes after the Plan Generator's generation of a new DAG plan or after the rePlanner's partial execution plan. If validation succeeds, the plan is forwarded to the Plan Executor for execution; otherwise, the validator sends feedback back to the RePlanner for iterative refinement. This mechanism is critical for two reasons:

% 1. Error Prevention – It prevents the plan executor from executing unsound DAG paths.

% 2. Efficiency – It eliminates redundant execution attempts, along with avoiding spills into infinite loops or invalid tool outputs.

% The validation process comprises two components 1) Structural Validator – It verifies the syntactic and structural correctness of the generated plan against the database schema relationships. and 2) Semantic Validator – It verifies the semantic relevance and consistency of the sub-queries.

% The validated plan is passed to the Plan Executor if correctness is achieved; otherwise, the feedback-form correction is reported for adaptive replanning.

% % \input{structural_validator}

% \subsubsection{Structural Validator}
% \label{subsec:strc_validator}

% % This subsection of the Plan Validator explains about validating the structural aspects of the plan generated by the plan generator on checking whether all the fields required are being persisted and if the dag plan has any cyclic dependencies or used a column name that is not present in the given schema. 

% % This is the continuation
% \begin{algorithm}
% \caption{Execution Plan Validation}
% \begin{algorithmic}[1]

% \Require $S$ \Comment{Database schema}
% \Require $P$ \Comment{Execution plan with list P.subquestions}

% \Statex
% \Comment{\textbf{1. Plan Structural Specification}}
% \If{subquestions not in P or not list P.subquestions}
%     \State \textbf{Error}
% \EndIf

% \For{each $q_i$ in P.subquestions, $i = 1 \dots n$}
%     \If{$q_i.status$ equals executed}
%         \State \textbf{Continue}
%     \EndIf
%     \State Require question, tool, label, and should\_expose\_answer exist
%     \State Assert question is non-empty string
%     \State Assert tool is iceberg or milvus
%     \State Assert label matches \texttt{\$var\_int}
%     \State Assert should\_expose\_answer is Boolean
%     \If{should\_expose\_answer equals TRUE}
%         \State Require answer\_description is non-empty
%     \EndIf
% \EndFor

% \State Require there exists $q_i$ with should\_expose\_answer equals TRUE

% \Statex
% \Comment{\textbf{2. Dependency-Expression Hygiene}}
% \State Pattern gets \texttt{\$var\_d[.c]}

% \For{each non-executed $q_i$}
%     \For{each match (v\_d, c) in question}
%         \State $d$ gets integer after \texttt{\$var\_}
%         \If{$d > n$}
%             \State \textbf{Error: Unknown variable}
%         \EndIf
%         \If{$c \neq \varnothing$ and $c$ not in $S$ and $c$ not in partialResult[\texttt{\$var\_d}]}
%             \State \textbf{Error: Unknown column}
%         \EndIf
%     \EndFor
% \EndFor

% \Statex
% \Comment{\textbf{3. Acyclic Intralogic Dependencies}}
% \State Build directed graph $G$
% \State Nodes get labels of $q_i$ without leading \texttt{\$}
% \State Edge $(u \to v)$ if $q_u$ references variable \texttt{\$var\_v}
% \If{DFS detects cycle in $G$}
%     \State \textbf{Error: Cyclic dependency}
% \EndIf

% \Statex
% \Comment{\textbf{4. Result}}
% \State VALID gets true if no errors recorded
% \State Output validation: VALID, feedback: list\_of\_errors

% \end{algorithmic}
% \end{algorithm}

% The Structural Validator ensures the syntactic correctness of a generated DAG plan $P$ compared to the schema $S$, verifying format compliance, referencing integrity, and dependency hygiene. Our validation logic for the sub-queries and schema references can be formalized as:

% $V_{struct}: (P,S) \rightarrow (structurally_valid,feedback)$

% where, $structurally_valid$ is a boolean flag to signify absence of structural errors. Feedback is a collection of structural errors and other proposer corrections.

% First, it cross-references if each of the nodes in P.subquestions are indeed part of the ongoing P. It interacts with the nodelist for each task, ensuring the attributes exist as shown in the Algorithm 1. While the question needs to be non-empty, the tool can be either $\{iceberg or milvus\}$. A clearly defined configuration of should\_expose\_answer is declared to ensure the proposal does exist in the post-try naming convention along with the compliance for the answer\_description, when the should\_expose\_answer = TRUE.

% Next, the missing intermediate variable referencing is tracked. It cross checks label parity followed by the PartialResults conciliation, altogether has to be formatted as \$var\_d.colname. For consistency, a manual cross-check against P.subquestions functioning with respect to P->subquestions in the schedule is executed using a DFS search for cyclic dependency AA.

% Finally, all the validation corrections are logged into the list\_of\_errors after collating the present status and feedback to the RePlanner for revision. After the validation is done the clean status is passed back to the Plan Executor for the final execution of the query. Refer to Algorithm 1 for the structural validator’s formal representation.

% % \input{semantic_validator}

% \subsubsection{Semantic Validator}
% \label{subsec:sem_validator}

% The semantic validator $V_{semantic}$ checks for coverage, accuracy, compliance, and optimization feasibility for the generated DAG plan before sending it off for final execution. While structure validator's rules coverage sections can validate some syntax inconsistencies and programming language blocks, they cannot understand the nuances of intent correctness that originates due to changes in subquestion levels set for the obtained plan, especially the optimization discrepancies introduced as a result of cross-qualification semantics.

% The semantic validator takes care of this aspect completely. It cross-checks the logical consistency and exhaustiveness in all subqueries. The input of this module is the database schema $S$ along with the execution plan $P$ and is resolved as: 

% $V_{semantic}:(P,S) \rightarrow {(validation:VALID, feedback:list of errors)}$

% Our semantic validator leverages only open-source LLMs for the validation of the plan by using a specialized plan-outlining prompt template. Once the plan passes the structural validation, the semantic validator checks for the optimized way of plan reorganizations and improvements. Detailed plan modification feedback, if present from the LLM is taken to re-planners for optimal improvements. If no further violations are found the corresponding validated plan is finally sent to the Plan Executor.



% \subsection{Replanner}
% \label{subsec:plan_validator}

% The Replanner Module is a crucial component that adapts the execution plan based on feedback received from various stages of processing, ensuring robustness and accuracy in query execution. We define the replanning process as:
% $Replanner (P,S,H,F) \rightarrow P'$ 
% where:
% $P$ is the original or partially executed plan.
% $S$ is the database schema.
% $H$ is the history of previous replanning attempts for the query.
% $F$ is the feedback received from validators or the plan executor.
% $P'$ is the refined or updated plan.

% The Replanner is an intelligent system that revises the execution plan based on feedback from the Structural Validator, Semantic Validator, and Plan Executor. It maintains a history of previous changes made to a query, allowing it to make informed decisions during replanning. It is essential for handling runtime errors, validation failures, and execution inconsistencies. It ensures that the system can recover from failures and adapt to changing conditions without restarting the entire query processing pipeline.

% The Replanner consists of two primary submodules:

% 1. \textbf{Fixer} – A lightweight submodule that quickly addresses variable dependency errors at the subquery level. It modifies only the affected subquery, minimizing latency.

% 2. \textbf{Worker} – A more comprehensive submodule that handles complex feedback requiring significant changes to the DAG plan. While it may introduce higher latency, it improves overall performance by addressing deeper issues.

% The Replanner operates conditionally, ensuring that already executed subqueries remain unchanged to preserve valid intermediate results. By intelligently revising the plan based on feedback and historical context, the Replanner enhances the system's resilience and adaptability.



% % \input{fixers}

% \subsubsection{Fixer}
% \label{subsec:fixer}

% The Fixer is a lightweight submodule within the Replanner that specializes in quick fixes for issues that affect a single node in the DAG plan without altering the overall structure. It leverages an LLM-based refinement approach to address feedback from the Plan Executor or Validators.

% One common scenario where the Fixer is useful is when a variable dependency error occurs during execution. For instance, consider the DAG plan in Figure 2:

% Subquery 1: Retrieves document\_id for a specific event.
% Subquery 2: Fetches the name and ID of the athlete using $\$var\_1$.document\_id. However, the SQL execution may rename the document\_id column to id in the result.
% Subquery 3: Tries to access $\$var\_2$.document\_id, but since document\_id is not present in $\$var\_2$ (only name and id are), a dependency error occurs.

% The Fixer intervenes by rewriting Subquery 3 to use id instead of document\_id, ensuring compatibility with the output of Subquery 2. This is achieved through an LLM that analyzes the feedback, the dependent query results, and the current query, generating a revised subquery that resolves the dependency issue.

% % \input{replanner_module}

% \subsubsection{Worker}
% \label{subsec:replanner_worker}

% The Worker is the core component of the Replanner, designed to handle complex feedback from various modules within the system. It leverages an LLM to analyze the feedback, along with the history of previous attempts, the current plan, the user query, the database schema, and any available execution results.

% The Worker addresses a wide range of issues, including:
% 1. Structural Validation Failures: When the plan does not conform to the required DAG structure, the Worker revises the plan to ensure it meets the necessary structural criteria.

% 2. Semantic Validation and Optimization: The Worker optimizes the plan for better performance, addressing any semantic issues or missed aspects that could impact execution.

% 3. Execution Errors: The Worker handles SQL execution errors and Milvus execution errors by rephrasing queries, breaking them down into simpler subqueries, or adjusting the query logic to avoid errors.

% The Worker operates by conducting a comprehensive analysis of the entire context, including the user query, database schema, and execution history. It uses an LLM-driven refinement approach to generate a revised plan that addresses identified issues while preserving the results of already executed subqueries. This process involves adaptive replanning, where the Worker focuses on refining failed and pending subqueries to ensure the revised plan is optimized for execution.

% \subsection{Plan Executor}
% \label{subsec:plan_executor}

% The Plan Executor Module is the final stage in the A.DOT pipeline, responsible for executing sub-queries following the DAG-approved plan to produce the final output. This component accepts the validated plan and systematically processes the queries as per the DAG generation privilege, keeping track of already executed sub-queries and immediately returns partial answers to the user.

% A key challenge in the Plan Executor is the effective passing of sub-query results of large enterprise datasets, which often contain sizes of details in the thousands. For instance, consider the scenario in the DAG illustrated in the figure 2, where the third sub-query, “What year was the athlete with document\_id in $\$var2.document_id$ born?”, depends on the document\_ids generated by the second sub-query. This dependency resolution implicates sending such extensive column-diversion results directly being heavy on resources and potentially leading to errors.

% To overcome this, the system first slims down the keys of if-interdependent variable queries to perform sample query replacements. It dynamically shrinks the scope of variable dependencies (e.g., document\_ids injected into a query retrieving birth years) without injecting the full payload into the variable. This approach optimizes query execution and avoids infrastructural bottlenecks.

% Once the dependency slimming is done, it transitions to database-instructive processing:

% 1. For SQL tables: The query is converted into an executable SQL statement using the Text2SQL module, recovered through heuristic knowledge-perform adjustments.

% 2. For Milvus documents: The corresponding Text2Milvus laser-document model converts the query into a vector embeddings-specific query and follows a dense and sparse retrieval phase, leveraging the document\_id to metadata tags mappings.

% Post-conversion, sample filter values in generated queries are replaced with full dataset values for optimal retrieval. Finally, the Plan Executor follows a streaming-like execution mechanism, utilizing the should\_expose\_answer flag by immediately showing answers that can be independently generated to the user. A user sees the completion of the answer stream only when all sub-queries linking full dependencies to usubstantial truths are completed. In the event of Milvus or Iceberg execution failure, feedback comprising the query execution status and partial results is sent to the Replanner for adaptive refinement and full success redemption repetition.

% Finally, the Answer Generator compresses the results from different executed subqueries to produce the final synthesized answer based on all sub-query executions, preserving the chain of confidence through the evaluated computation.

% \input{overview}

% \input{database_construction}

% \input{plan_caching}

% \input{plan_generator}

% \input{plan_validator}

% \input{replanner}

% \input{plan_executor}

==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}

The subsections is not decided yet, but i have in mind of comparing with the existing hybridqa based table and text answering, and the agentic frameworks that tries to handle the realtime multihop question answering and comparing our work with these.

==> replanner_module.tex <==
\subsubsection{Worker}
\label{subsec:replanner_worker}

The Worker is the core component of the Replanner, designed to handle complex feedback from various modules within the system. It leverages an LLM to analyze the feedback, along with the history of previous attempts, the current plan, the user query, the database schema, and any available execution results.

The Worker addresses a wide range of issues, including:
1. Structural Validation Failures: When the plan does not conform to the required DAG structure, the Worker revises the plan to ensure it meets the necessary structural criteria.

2. Semantic Validation and Optimization: The Worker optimizes the plan for better performance, addressing any semantic issues or missed aspects that could impact execution.

3. Execution Errors: The Worker handles SQL execution errors and Milvus execution errors by rephrasing queries, breaking them down into simpler subqueries, or adjusting the query logic to avoid errors.

The Worker operates by conducting a comprehensive analysis of the entire context, including the user query, database schema, and execution history. It uses an LLM-driven refinement approach to generate a revised plan that addresses identified issues while preserving the results of already executed subqueries. This process involves adaptive replanning, where the Worker focuses on refining failed and pending subqueries to ensure the revised plan is optimized for execution.
